WAVES: Benchmarking the Robustness of Image Watermarks

In the burgeoning age of generative AI, watermarks act as identifiers of provenance and artificial content. We present WAVES (Watermark Analysis Via Enhanced Stress-testing), a benchmark for assessing image watermark robustness, overcoming the limitations of current evaluation methods. WAVES integrates detection and identification tasks and establishes a standardized evaluation protocol comprised of a diverse range of stress tests. The attacks in WAVES range from traditional image distortions to advanced, novel variations of diffusive, and adversarial attacks. Our evaluation examines two pivotal dimensions: the degree of image quality degradation and the efficacy of watermark detection after attacks. Our novel, comprehensive evaluation reveals previously undetected vulnerabilities of several modern watermarking algorithms. We envision WAVES as a toolkit for the future development of robust watermarks. The project is available at https://wavesbench.github.io/

==> figures/2x_regen_diffusion.tex <==
\begin{figure}[!htbp]
  \centering
  \subcaptionbox{2x\_Regen-20}{\includegraphics[width=0.22\linewidth]{figures/regen_images/2x_regen-20.png}}
  \subcaptionbox{2x\_Regen-60}{\includegraphics[width=0.22\linewidth]{figures/regen_images/2x_regen-60.png}}
  \subcaptionbox{2x\_Regen-100}{\includegraphics[width=0.22\linewidth]{figures/regen_images/2x_regen-100.png}}
  \caption{2x rinsing regeneration with varying depth of noising steps per diffusion.}
  \label{fig:2x_regen_diffusion_three-subfigures}
\end{figure}

==> figures/regen_performance.tex <==
\begin{figure}[!htbp]
    \centering
    \hfil
    \begin{subfigure}{0.36\textwidth}
        \includegraphics[width=\linewidth]{figures/regen_diff_psnr.png}
        \caption{TPR@0.1\%FPR vs. PSNR ($\uparrow$)}
    \end{subfigure}
    \hfil
    \begin{subfigure}{0.36\textwidth}
        \includegraphics[width=\linewidth]{figures/regen_diff_clip.png}
        \caption{TPR@0.1\%FPR vs. CLIP-FID ($\downarrow$)}
    \end{subfigure}
    \hfil\\
    \hfil
    \begin{subfigure}{0.36\textwidth}
        \includegraphics[width=\linewidth]{figures/regen_coco_psnr.png}
        \caption{TPR@0.1\%FPR vs. PSNR ($\uparrow$)}
    \end{subfigure}
    \hfil
    \begin{subfigure}{0.36\textwidth}
        \includegraphics[width=\linewidth]{figures/regen_coco_clip.png}
        \caption{TPR@0.1\%FPR vs. CLIP-FID ($\downarrow$)}
    \end{subfigure}
    \hfil
    \caption{Regeneration attacks on the Tree-Ring watermark. Regen-Diff is a single diffusive regeneration and Rinse-[N]xDiff is a rinsing regeneration with $N$ repeated diffusions; the strengths indicate the number of noising steps in each diffusion. Regen-VAE uses a pre-trained VAE (bmshj2018) \cite{DBLP:conf/iclr/BalleMSHJ18} from the CompressAI library with quality factor as strength and Regen-KLVAE uses pre-trained KL-loss VAEs from the CompVis \cite{kingma2022autoencoding} with bottleneck size as strength. RinseD-VAE applies a VAE (bmshj2018) as a denoiser to Rinse-4xDiff attacked images. 2x rinsing and VAE regenerations are especially powerful against the Tree-Ring without extensively sacrificing image quality.}
    \label{multi-regen}
\end{figure}




==> icml_sec/6_conclusion.tex <==
\section{Conclusion}
In this work, we comprehensively assess the robustness of several popular watermarking techniques. Our framework, WAVES, uses a battery of attacks to degrade a watermark. The potency of an attack is jointly judged against two metrics: detection/identification probability of the watermark and quality of the image after the attack. We provide a taxonomy, categorization, and ranking of over 20+ styles of attack on the DiffusionDB, MS-COCO, and DALLE$\cdot$3 datasets. In particular, our normalized ranking of an attack's viability aggregates many popular perceptual metrics. Our analysis highlights the vulnerabilities of existing watermarking strategies. WAVES can serve as a practical field guide to the design and evaluation of any watermarking algorithm.  

\paragraph{Limitations.} We only stress-test the Tree-Ring, Stable Signature, and Stegastamp watermarking algorithms. We curated these watermarks for WAVES after an extensive literature review indicated these three techniques to be the most powerful and practical candidates for deployment in the wild. However, we emphasize our framework is extensible to any watermarking method.
Additionally, our attack ranking method relies on author-selected TPR thresholds and image quality metrics that we believe will fairly capture attack potency based on existing literature and experimental studies. The use of other quality metrics (MSE, Watson-DFT, etc.) and differing TPR thresholds may affect attack rankings.


==> include/000_premeable.tex <==
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{booktabs} 
\usepackage{multicol}
\usepackage{multirow}
\usepackage{ulem}
\usepackage{soul}
% \usepackage[labelfont=bf,textfont=bf,justification=centering]{caption}
\RequirePackage[format=plain,labelformat=simple,labelsep=period,font=small,compatibility=false]{caption}
\RequirePackage[font=footnotesize,skip=3pt,subrefformat=parens]{subcaption}

% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% \usepackage{smile}
\usepackage{comment}
\usepackage{url}
\usepackage{hyperref}

\newenvironment{colored}[1]{\leavevmode\color{#1}\ignorespaces}{}
\usepackage{amsmath}
\usepackage{amssymb} 
\usepackage{amsthm}
\usepackage{tabularx}
\usepackage{caption}
\usepackage{caption}
\usepackage{color}
% \captionsetup{justification=centering}

% \usepackage{xcolor}
% \usepackage[table]{xcolor}  % added by Sicheng
% \usepackage{soul}  % added by Sicheng, for strikethrough
\usepackage{bbm}

% Added by Sicheng
\usepackage{adjustbox} 
\usepackage{wrapfig}

\usepackage{mathtools}


\usepackage{siunitx}
\usepackage{etoolbox}
\sisetup{separate-uncertainty=true,detect-weight,table-format=2.2,table-figures-uncertainty=1}
\robustify\bfseries

\usepackage[T1]{fontenc}

% \renewcommand{\algorithmiccomment}[1]{#1}
% added by Sicheng
% \newcommand{\methodname}[1][]{$\mathtt{ReasoningCLIP}$}
% \newcommand{\methodname}{$\mathtt{PerceptionCLIP}$}
% \usepackage{algpseudocode}
% \usepackage{algorithm2e}
% \RestyleAlgo{ruled}
% \SetKwComment{Comment}{/* }{ */}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \SetKwInOut{Require}{Require}

\def \AdvRisk {\mathrm{AdvRisk}}
\def \Risk {\mathrm{Risk}}
\def \sgn {\mathrm{sgn}}
% \def \Ball {\mathrm{Ball}}
% \def \bin {\text{bin}}

\newcommand{\facc}[2]{{#1}{\scriptsize±{#2}}}
\newcommand{\bfacc}[2]{\textbf{{#1}{\scriptsize±{#2}}}} % added by sicheng
\usepackage[toc,page,header]{appendix}
\usepackage{minitoc}
% Make the "Part I" text invisible
\renewcommand \thepart{}
\renewcommand \partname{}
\newcommand{\ind}{\perp\!\!\!\perp} 
% \newcommand{\ind}{\perp\!\!\!\!\perp} 


\newcommand\shortsection[1]{\vspace{0pt}{\noindent\bf #1}}

\DeclareMathOperator{\esssup}{{\rm -ess\:sup}}

\newcommand{\largeabstract}{\large}  % Change '\large' to the desired font size

\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage{enumitem}
\newlist{parenum}{enumerate}{1}
\setlist[parenum,1]{label=\textbf{(\arabic*)}, wide, labelwidth=!, labelindent=0pt, topsep=0pt, itemsep=-1ex, partopsep=0ex, parsep=1ex}

\usepackage{adjustbox}
\usepackage[para,online,flushleft]{threeparttable}


==> include/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> table/attack_summary.tex <==

\begin{table*}[t]
\caption{A taxonomy of all the attacks in our stress-testing set.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Category}}     & \textbf{Subcategory}                        & \multirow{2}{*}{\textbf{Description}}         & \textbf{Attack Names}                                                & \multirow{2}{*}{\textbf{Requirements}}                                       \\ 
                              & \textbf{(prefix)}                          &                                      & \textbf{(suffix)}                                                    &        \\
\midrule
\multirow{4}{*}{Distortion}   & Single     & \multirow{2}{*}{Single distortion}   & -Rotation, -RCrop, -Erase, -Bright,                             & \multirow{2}{*}{-}      \\
                              & (Dist-)                                   &                                      & -Contrast, -Blur, -Noise, -JPEG                                 &                       \\\cline{2-5} 
                              & Combination & Combination of  & -Geo, -Photo,                                                & \multirow{2}{*}{-}    \\
                              & (DistCom-) &   a type of distortions                                   & -Deg, -All                                                    &                                       \\
\midrule
\multirow{4}{*}{Regeneration} & Single   &  A single VAE or     & -Diff, -DiffP    & DiffP requires user prompts \\
                              & (Regen-)          &  diffusion regeneration                                    &  -VAE, -KLVAE                                                           &  KLVAE with bottleneck size 8 is grey-box                                    \\\cline{2-5} 
                              & Rinsing    &  A multi-diffusion       & \multirow{2}{*}{-2xDiff, -4xDiff}     & \multirow{2}{*}{-} \\
                              & (Rinse-)    &  regeneration       &     &   
\midrule
\multirow{6}{*}{Adversarial}  & Embedding (grey-box) & \multirow{2}{*}{Use the same VAE} & \multirow{2}{*}{-KLVAE8}                                                      & \multirow{2}{*}{grey-box}    \\
                              & (AdvEmbG-)                                   &                                      &                                                             &                                 \\\cline{2-5} 
                              & Embedding (black-box) & \multirow{2}{*}{Use other encoders} & -RN18, -CLIP,                                                & \multirow{2}{*}{-}       \\
                              & (AdvEmbB-)                                   &                                      & -KLVAE16, -SdxlVAE                                            &                                        \\\cline{2-5} 
                              & Surrogate detector attack  & \multirow{2}{*}{Train a watermark detector} & -UnWM\&WM, -Real\&WM,                                       & \multirow{2}{*}{need data and training}    \\
                              &  (AdvCLS-)                                  &                                      & -WM1\&WM2                                                    &                               \\
\bottomrule
\end{tabular} \label{tab:summary_attacks}
}
\end{table*}

